Gaming security by obscurity

Shannon sought security against the attacker with unlimited computational powers: *if an information source conveys some information, then Shannon's attacker will surely extract that information*. Diffie and Hellman refined Shannon's attacker model by taking into account the fact that the real attackers are computationally limited. This idea became one of the greatest new paradigms in computer science, and led to modern cryptography. Shannon also sought security against the attacker with unlimited logical and observational powers, expressed through the maxim that "the enemy knows the system". This view is still endorsed in cryptography. The popular formulation, going back to Kerckhoffs, is that "there is no security by obscurity", meaning that the algorithms cannot be kept obscured from the attacker, and that security should only rely upon the secret keys. In fact, modern cryptography goes even further than Shannon or Kerckhoffs in tacitly assuming that *if there is an algorithm that can break the system, then the attacker will surely find that algorithm*. The attacker is not viewed as an omnipotent computer any more, but he is still construed as an omnipotent programmer. So the Diffie-Hellman step from unlimited to limited computational powers has not been extended into a step from unlimited to limited logical or programming powers. Is the assumption that all feasible algorithms will eventually be discovered and implemented really different from the assumption that everything that is computable will eventually be computed? The present paper explores some ways to refine the current models of the attacker, and of the defender, by taking into account their limited logical and programming powers. If the adaptive attacker actively queries the system to seek out its vulnerabilities, can the system gain some security by actively learning attacker's methods, and adapting to them?

==> PICS/trust-net.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 03 15:59:25 PST 2010
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="110" y-min="3" y-max="87" auto-bounding="true">
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(22,81);(22,81);(96,14);(96,14)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<parallelogram p3= "(102,57)"
%	 fill-color= "#0000ff"
%	 p2= "(102,53)"
%	 p1= "(98,53)"
%	 fill-style= "solid"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,47)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,43)"
%	 p1= "(18.5,43)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(102,37)"
%	 fill-color= "#0000ff"
%	 p2= "(102,33)"
%	 p1= "(98,33)"
%	 fill-style= "solid"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram p3= "(102,77)"
%	 fill-color= "#0000ff"
%	 p2= "(102,73)"
%	 p1= "(98,73)"
%	 fill-style= "solid"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,67)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,63)"
%	 p1= "(18.5,63)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,85.62);(23.12,85.62);(95.62,76.88);(95.62,76.88)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,64.38);(23.12,64.38);(96.25,56.25);(96.25,56.25)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "1.1"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,62.5);(23.12,62.5);(96.25,36.88);(96.25,36.88)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(30,59)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\five$
%</text>
%<ellipse p3= "(21.5,87)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,83)"
%	 p1= "(18.5,83)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,27)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,23)"
%	 p1= "(18.5,23)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23,82);(23,82);(95,40);(95,40)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(22.5,6.88);(22.5,6.88);(96.88,51.88);(96.88,51.88)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,46.88);(23.12,46.88);(96.25,73.12);(96.25,73.12)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.38,45.12);(23.38,45.12);(96.25,55);(96.25,55)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.85"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.75,65.62);(23.75,65.62);(96.62,74.38);(96.62,74.38)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,23.75);(23.12,23.75);(96.25,33.75);(96.25,33.75)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,26.88);(23.12,26.88);(96.88,71.25);(96.88,71.25)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.38,25.12);(23.38,25.12);(96.25,53.75);(96.25,53.75)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(30,50.62)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\six$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(42.5,48.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\seven$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(30,41.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eight$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(29.38,31.25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\nine$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(31.88,23.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eleven$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(48.12,34.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ten$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,85)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ha$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,65)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hb$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,45)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hc$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,25)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hd$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hI$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,55)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hII$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,35)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIII$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(30,86)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(29.38,67.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<parallelogram p3= "(102,17)"
%	 fill-color= "#0000ff"
%	 p2= "(102,13)"
%	 p1= "(98,13)"
%	 fill-style= "solid"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,7)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,3)"
%	 p1= "(18.5,3)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,3.75);(23.12,3.75);(96.88,13.75);(96.88,13.75)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\he$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,15)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIV$
%</text>
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23,84);(23,84);(96.25,57.5);(96.25,57.5)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,43.75);(23.12,43.75);(96.26,35.63);(96.26,35.63)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,5.62);(23.12,5.62);(96.88,32.5);(96.88,32.5)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(30,11.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\twelve$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(30.62,3.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fourteen$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(44.38,12.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\thirteen$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(25,78)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\fifteen$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(50,75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\two$
%</text>
%<text text-vert-align= "baseline"
%	 anchor-point= "(38.12,73.75)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\sixteen$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(46.88,62.5)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,87)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22,81)(96,14)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,53)(102,53)(102,57)(98,57)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,45){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,33)(102,33)(102,37)(98,37)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,73)(102,73)(102,77)(98,77)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,85.62)(95.62,76.88)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,64.38)(96.25,56.25)
\psline[border=1.1,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,62.5)(96.25,36.88)
\rput[t](30,59){$\five$}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,85){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,82)(95,40)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22.5,6.88)(96.88,51.88)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,46.88)(96.25,73.12)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,45.12)(96.25,55)
\psline[border=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.75,65.62)(96.62,74.38)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,23.75)(96.25,33.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,26.88)(96.88,71.25)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,25.12)(96.25,53.75)
\rput[b](30,50.62){$\six$}
\rput[b](42.5,48.75){$\seven$}
\rput[t](30,41.25){$\eight$}
\rput[br](29.38,31.25){$\nine$}
\rput[t](31.88,23.75){$\eleven$}
\rput[tl](48.12,34.38){$\ten$}
\rput(10,85){$\ha$}
\rput(10,65){$\hb$}
\rput(10,45){$\hc$}
\rput(10,25){$\hd$}
\rput(110,75){$\hI$}
\rput(110,55){$\hII$}
\rput(110,35){$\hIII$}
\rput[b](30,86){$\one$}
\rput[b](29.38,67.5){$\three$}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,13)(102,13)(102,17)(98,17)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,5){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,3.75)(96.88,13.75)
\rput(10,5){$\he$}
\rput(110,15){$\hIV$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,84)(96.25,57.5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,43.75)(96.26,35.63)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,5.62)(96.88,32.5)
\rput[br](30,11.88){$\twelve$}
\rput[t](30.62,3.75){$\fourteen$}
\rput[tl](44.38,12.5){$\thirteen$}
\rput[tr](25,78){$\fifteen$}
\rput[bl](50,75){$\two$}
\rput[Bl](38.12,73.75){$\sixteen$}
\rput[b](46.88,62.5){$\four$}
\end{pspicture}


==> PICS/trust-recommend.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Fri Dec 03 15:59:40 PST 2010
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="110" y-min="8" y-max="72" auto-bounding="true">
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(65,51.88);(65,51.88);(96.25,60);(96.25,60)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23,69);(23,69);(56,54);(56,54)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<parallelogram p3= "(102,42)"
%	 fill-color= "#0000ff"
%	 p2= "(102,38)"
%	 p1= "(98,38)"
%	 fill-style= "solid"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram p3= "(102,22)"
%	 fill-color= "#0000ff"
%	 p2= "(102,18)"
%	 p1= "(98,18)"
%	 fill-style= "solid"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram p3= "(102,62)"
%	 fill-color= "#0000ff"
%	 p2= "(102,58)"
%	 p1= "(98,58)"
%	 fill-style= "solid"
%	 stroke-color= "#0000ff"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(65,30);(65,30);(96.88,38.12);(96.88,38.12)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(27,52)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\two$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(27,28)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\five$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(28,68)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(27,18)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\six$
%</text>
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(64.38,32.5);(64.38,32.5);(96.25,58.12);(96.25,58.12)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(65,48.12);(65,48.12);(96.88,40.62);(96.88,40.62)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(64.38,27.5);(64.38,27.5);(96.25,20);(96.25,20)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<text text-vert-align= "bottom"
%	 anchor-point= "(90,59.38)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eight$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,60)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hI$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,40)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hII$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(110,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIII$
%</text>
%<ellipse p3= "(21.5,32)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,28)"
%	 p1= "(18.5,28)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,52)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,48)"
%	 p1= "(18.5,48)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,72)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,68)"
%	 p1= "(18.5,68)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,12)"
%	 fill-color= "#ff6666"
%	 p2= "(21.5,8)"
%	 p1= "(18.5,8)"
%	 closure= "open"
%	 fill-style= "solid"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,70)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ha$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hb$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hc$
%</text>
%<text text-vert-align= "center-v"
%	 anchor-point= "(10,10)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hd$
%</text>
%<parallelogram p3= "(60.23,54.33)"
%	 stroke-width= "0.55"
%	 p2= "(56.5,50.06)"
%	 p1= "(59.77,45.67)"
%	 fill-style= "none"
%	 stroke-color= "#660099"
%	 />
%<parallelogram p3= "(60.23,34.33)"
%	 stroke-width= "0.55"
%	 p2= "(56.5,30.06)"
%	 p1= "(59.77,25.67)"
%	 fill-style= "none"
%	 stroke-color= "#660099"
%	 />
%<multicurve arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23,29);(23,29);(55,29);(55,29)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.9"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23,51);(23,51);(55,51);(55,51)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.9"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23,49);(23,49);(55,32);(55,32)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.9"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23,31);(23,31);(56,48);(56,48)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(22.5,11.88);(22.5,11.88);(56.88,45.62);(56.88,45.62)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<multicurve stroke-overstrike= "true"
%	 stroke-overstrike-width= "0.75"
%	 arrow-head-width-minimum= "1.45"
%	 right-arrow= "head"
%	 arrow-head-length-scale= "1.55"
%	 fill-style= "none"
%	 points= "(23.12,9.38);(23.12,9.38);(55.62,26.25);(55.62,26.25)"
%	 arrow-global-scale-length= "1.45"
%	 />
%<text text-vert-align= "top"
%	 anchor-point= "(30,12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\seven$
%</text>
%<text text-vert-align= "bottom"
%	 anchor-point= "(27,34)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "top"
%	 anchor-point= "(27,46)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<text text-vert-align= "bottom"
%	 stroke-width= "0.5"
%	 anchor-point= "(91,43)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\nine$
%</text>
%<text text-vert-align= "top"
%	 stroke-width= "0.5"
%	 anchor-point= "(91.88,53.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ten$
%</text>
%<text text-vert-align= "top"
%	 stroke-width= "0.5"
%	 anchor-point= "(91,36)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eleven$
%</text>
%<text text-vert-align= "top"
%	 stroke-width= "0.5"
%	 anchor-point= "(90,20)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\twelve$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(60,50)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\Three$
%</text>
%<text text-vert-align= "center-v"
%	 stroke-width= "0.5"
%	 anchor-point= "(60,30)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\One$
%</text>
%<text text-vert-align= "bottom"
%	 stroke-width= "0.5"
%	 anchor-point= "(60,56.88)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\concone$
%</text>
%<text text-vert-align= "top"
%	 stroke-width= "0.5"
%	 anchor-point= "(60,23.12)"
%	 fill-style= "none"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\conctwo$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,72)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(65,51.88)(96.25,60)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,69)(56,54)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,38)(102,38)(102,42)(98,42)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,18)(102,18)(102,22)(98,22)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,58)(102,58)(102,62)(98,62)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(65,30)(96.88,38.12)
\rput[b](27,52){$\two$}
\rput[t](27,28){$\five$}
\rput[b](28,68){$\one$}
\rput[b](27,18){$\six$}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(64.38,32.5)(96.25,58.12)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(65,48.12)(96.88,40.62)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(64.38,27.5)(96.25,20)
\rput[b](90,59.38){$\eight$}
\rput(110,60){$\hI$}
\rput(110,40){$\hII$}
\rput(110,20){$\hIII$}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,30){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,50){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,70){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,10){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\rput(10,70){$\ha$}
\rput(10,50){$\hb$}
\rput(10,30){$\hc$}
\rput(10,10){$\hd$}
\newrgbcolor{userLineColour}{0.4 0 0.6}
\pspolygon[linewidth=0.55,linecolor=userLineColour](59.77,45.67)(56.5,50.06)(60.23,54.33)(63.5,49.94)
\newrgbcolor{userLineColour}{0.4 0 0.6}
\pspolygon[linewidth=0.55,linecolor=userLineColour](59.77,25.67)(56.5,30.06)(60.23,34.33)(63.5,29.94)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,29)(55,29)
\psline[border=0.9,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,51)(55,51)
\psline[border=0.9,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,49)(55,32)
\psline[border=0.9,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,31)(56,48)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22.5,11.88)(56.88,45.62)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,9.38)(55.62,26.25)
\rput[t](30,12){$\seven$}
\rput[b](27,34){$\four$}
\rput[t](27,46){$\three$}
\rput[b](91,43){$\nine$}
\rput[t](91.88,53.12){$\ten$}
\rput[t](91,36){$\eleven$}
\rput[t](90,20){$\twelve$}
\rput(60,50){$\Three$}
\rput(60,30){$\One$}
\rput[b](60,56.88){$\concone$}
\rput[t](60,23.12){$\conctwo$}
\end{pspicture}

